Electronics and data acquisition demonstrator for a kinetic inductance camera

A prototype of digital frequency multiplexing electronics allowing the real time monitoring of kinetic inductance detector (KIDs) arrays for mm-wave astronomy has been developed. It requires only 2 coaxial cables for instrumenting a large array. For that, an excitation comb of frequencies is generated and fed through the detector. The direct frequency synthesis and the data acquisition relies heavily on a large FPGA using parallelized and pipelined processing. The prototype can instrument 128 resonators (pixels) over a bandwidth of 125 MHz. This paper describes the technical solution chosen, the algorithm used and the results obtained.

==> Makefile <==
FICHIER_TEX= article_KID.tex
ARCHIVE=$(FICHIER_TEX:%.tex=%.zip)


all : 
	pdflatex ${FICHIER_TEX}
################################################
#lance le make de chaque sous rep

clean: $(REP)
	@echo "suppression des fichiers de compilation"
	@# fichiers de compilation latex
	@rm -f *.log *.aux *.dvi *.toc *.lot *.lof *.out
	@# fichiers de bibtex
	@rm -f *.bbl *.blg
	@# fichier zip 
	@rm -f *.zip

zip: 
	#rm ${ARCHIVE}
	grep includegraphics *.tex > liste.txt
	awk  '{st=index($$0,"{");rem=substr($$0,st+1); st=index(rem,"}"); rem=substr(rem,1,st-1); printf("zip -r ${ARCHIVE} %s.p*\nzip -r ${ARCHIVE} %s.j*\n",rem,rem);}' liste.txt > zip_liste.sh
	zip -r ${ARCHIVE} Makefile
	zip -r ${ARCHIVE} *.cls
	zip -r ${ARCHIVE} *.tex
	bash zip_liste.sh

